Saturable absorption in NV-doped diamond studied by femtosecond Z-scan

We investigate nonlinear optical absorption in diamond crystals containing high densities of nitrogen vacancy (NV) centers using open-aperture Z-scan measurements with 230 fs laser pulses at 1032 nm, within the transparency window of diamond. While high-purity electronic-grade diamond exhibits third-order nonlinear absorption, NV-doped samples display pronounced saturable absorption that strengthens with increasing defect concentration. Linear transmission spectroscopy reveals that, in addition to NV centers, the crystals host significant populations of H2 (NVN-) defect complexes whose absorption band partially overlaps the excitation wavelength. By correlating spectroscopic data with nonlinear measurements and modeling the response using an effective two-level system, we show that the observed saturation cannot be attributed solely to NV centers but arises from the combined contribution of NV-related and H2 defects. For the highly doped sample, we determine an effective linear absorption coefficient of alpha0 = 6.52 cm-1 and a saturation intensity of Is = 40.0 GW/cm2. These findings highlight the critical role of the complex defect landscape in governing the nonlinear optical response of NV-doped diamond and underscore the necessity of accounting for ancillary defect species in the design of diamond-based nonlinear and quantum photonic devices.

==> bib-copy.tex <==
@article{Abulikemu_2021,
    title  = {Second-Harmonic Generation in Bulk Diamond Based on Inversion Symmetry Breaking by Color Centers},
    author = {Aizitaili Abulikemu and Yuta Kainuma and Toshu An and Muneaki Hase},
    journal = {ACS Photonics},
    volume = {8},
    issue = {},
    pages = {988--993},
    numpages = {},
    year = {2021},
    month = {},
    publisher = {American Chemical Society},
    doi = {10.1021/acsphotonics.0c01806},
    url = {}
}

@article{Abulikemu_2022,
    title  = {Temperature-dependent second-harmonic generation from color centers in diamond},
    author = {Aizitiali Abulikemu and Yuta Kainuma and Tosku An and Muneaki Hase},
    journal = {Opt. Lett.},
    volume = {47},
    issue = {7},
    pages = {1693--1696},
    numpages = {},
    year = {2022},
    month = {},
    publisher = {Optica Publishing Group},
    doi = {10.1364/OL.455437},
    url = {}
}

@article{Abulikemu_2023,
    title  = {Highly-efficient third-harmonic generation from ultrapure diamond crystals},
    author = {Abulikemu A. and Hase M.},
    journal = {Optical Materials Express},
    volume = {13},
    issue = {4},
    pages = {916--924},
    numpages = {},
    year = {2023},
    month = {Apr},
    publisher = {Optica Publishing Group},
    doi = {10.1364/OME.485601},
    url = {}
}

@article{Acosta_2009,
    title  = {Diamonds with a high density of nitrogen-vacancy centers for magnetometry applications},
    author = {Acosta, V. M. and Bauch, E. and Ledbetter, M. P. and Santori, C. and Fu, K.-M. C. and Barclay, P. E. and Beausoleil, R. G. and Linget, H. and Roch, J. F. and Treussart, F. and Chemerisov, S. and Gawlik, W. and Budker, D.},
    journal = {Phys. Rev. B},
    volume = {80},
    issue = {11},
    pages = {115202},
    numpages = {15},
    year = {2009},
    month = {Sep},
    publisher = {American Physical Society},
    doi = {10.1103/PhysRevB.80.115202},
    url = {https://link.aps.org/doi/10.1103/PhysRevB.80.115202}
}

@article{Almeida_2017,
    title  = {Nonlinear optical spectrum of diamond at femtosecond regime},
    author = {Almeida, J.M.P. and Oncebay, C. and Sigueira, J.P. and Muniz, S.R. and DeBoni, L. and Mendonca, C.R.},
    journal = {Sci. Rep.},
    volume = {7},
    issue = {},
    pages = {14320},
    numpages = {},
    year = {2017},
    month = {Oct},
    publisher = {American Physical Society},
    doi = {10.1038/s41598-017-14748-4},
    url = {}
}

@article{Ardagozen_2014,
    title = {Wear of ultrananocrystalline diamond AFM tips during mechanical nanomanufacturing by nanomilling},
    journal = {Wear},
    volume = {317},
    number = {1},
    pages = {39-55},
    year = {2014},
    issn = {0043-1648},
    doi = {https://doi.org/10.1016/j.wear.2014.04.024},
    url = {https://www.sciencedirect.com/science/article/pii/S004316481400163X},
    author = {B. {A. Gozen} and O. {B. Ozdoganlar}},
    keywords = {Diamond, CVD coatings, AFM, Wear testing, Cutting tools},
}

@article{Balasubramanian_2014,
    title = {Nitrogen-Vacancy color center in diamond—emerging nanoscale applications in bioimaging and biosensing},
    journal = {Current Opinion in Chemical Biology},
    volume = {20},
    pages = {69-77},
    year = {2014},
    note = {Molecular imaging},
    issn = {1367-5931},
    doi = {https://doi.org/10.1016/j.cbpa.2014.04.014},
    url = {https://www.sciencedirect.com/science/article/pii/S1367593114000593},
    author = {Gopalakrishnan Balasubramanian and Andrii Lazariev and Sri Ranjini Arumugam and De-wen Duan},
}

@book{Boyd_2020,
    author    = {R. W. Boyd},
    title     = {Nonlinear Optics},
    year      = {2020},
    publisher = {Elsevier, London},
    isbn      = {978-0-323-85057-5},
}

@article{Buerki_1999,
    title = {Observation of the {H}2 defect in gem-quality type {I}a diamond},
    journal = {Diamond and Related Materials},
    volume = {8},
    number = {6},
    pages = {1061-1066},
    year = {1999},
    issn = {0925-9635},
    doi = {https://doi.org/10.1016/S0925-9635(99)00094-1},
    url = {https://www.sciencedirect.com/science/article/pii/S0925963599000941},
    author = {Peter R Buerki and Ilene M Reinitz and Sam Muhlmeister and Shane Elen},
    keywords = {H2 defect, Vacancy complexes, Annealing, Type Ia diamond, VIS–NIR spectrometry, Fancy color diamonds},

}

@article{Choe_2018,
    title = {Precise temperature sensing with nanoscale thermal sensors based on diamond NV centers},
    journal = {Current Applied Physics},
    volume = {18},
    number = {9},
    pages = {1066-1070},
    year = {2018},
    issn = {1567-1739},
    doi = {https://doi.org/10.1016/j.cap.2018.06.002},
    url = {https://www.sciencedirect.com/science/article/pii/S1567173918301573},
    author = {Sunuk Choe and Jungbae Yoon and Myeongwon Lee and Jooeon Oh and Dongkwon Lee and Heeseong Kang and Chul-Ho Lee and Donghun Lee},
    keywords = {Temperature sensing, Diamond NV center, Nanodiamond},
    
}

@article{Desalvo_1993,
    title  = {Z-scan measurements of the anisotropy of nonlinear refraction and absorption in crystals},
    author = {DeSalvo R. and Sheik_Bahae M. and Said A.A. and Hagan D.J. and Van Stryland E.W.},
    journal = {Opt. Letters},
    volume = {18},
    issue = {3},
    pages = {194--196},
    numpages = {},
    year = {1993},
    month = {Feb},
    publisher = {Optical Society of America},
    doi = {},
    url = {}
}

@article{Dhomkar_2016,
    title  = {Long-term data storage in diamond},
    author = {Dhomkar S. and Henshaw J. and Jayakumar H. and Meriles C.A.},
    journal = {Sci. Adv.},
    volume = {2},
    issue = {},
    pages = {e1600911},
    numpages = {},
    year = {2016},
    month = {},
    publisher = {American Association for the Advancement of Science},
    doi = {},
    url = {}
}

@article{Doherty_2013,
    author = {Doherty, Marcus W. and Manson, Neil B. and Delaney, Paul and Jelezko, Fedor and Wrachtrup, Jorg and Hollenberg, Lloyd C.L.}, 
    title = {The nitrogen-vacancy centre in diaomond},
    journal = {Physics Reports},
    volume = {528},  
    pages = {1-45},
    year = {2013},
    doi = {10.1016/j.physrep.2013.02.001}
}

@article{Dzierzega_2021,
    title  = {Optical nonlinearities of silicate oxide glass with gold nanoparticles outside the spectral range of surface plasmon resonance},
    author = {Krzysztof Dzierżęga and Aleksandra Wolak and Witold Zawadzki and Wojciech Talik and Nadia Pellerin and Babacar Diallo and Jean-Philippe Blondeau and Stephane Pellerin},
    journal = {Opt. Materials},
    volume = {122},
    issue = {},
    pages = {111712},
    numpages = {},
    year = {2021},
    month = {},
    publisher = {Elsevier},
    doi = {10.1016/j.optmat.2021.111712},
    url = {}
}

@article{Element6,
    title = {DNV B1 and DNV B14 Unlocking next generation quantum technologies},
    year = {2021},
    journal = {Element Six},
    doi = {https://www.sciencedirect.com/science/article/pii/S1357272520302132},
    author = {Element Six},
}

@article{filipkowski_2022,
    title = {Volumetric incorporation of NV diamond emitters in nanostructured F2 glass magneto-optical fiber probes},
    journal = {Carbon},
    volume = {196},
    pages = {10-19},
    year = {2022},
    issn = {0008-6223},
    doi = {https://doi.org/10.1016/j.carbon.2022.04.024},
    url = {https://www.sciencedirect.com/science/article/pii/S0008622322002949},
    author = {Adam Filipkowski and Mariusz Mrózek and Grzegorz Stępniewski and Jakub Kierdaszuk and Aneta Drabińska and Tanvi Karpate and Maciej Głowacki and Mateusz Ficek and Wojciech Gawlik and Ryszard Buczyński and Adam Wojciechowski and Robert Bogdanowicz and Mariusz Klimczak},
    keywords = {Diamond particles, Nitrogen-vacancy centers, Magnetic sensing, Optical fibers},
}

@article{Frantz_1963,
    author = {Frantz, Lee M. and Nodvik, John S.},
    title = {Theory of {P}ulse {P}ropagation in a {L}aser {A}mplifier},
    journal = {Journal of Applied Physics},
    volume = {34},
    number = {8},
    pages = {2346-2349},
    year = {1963},
    month = {08},
    issn = {0021-8979},
    doi = {10.1063/1.1702744},
    url = {https://doi.org/10.1063/1.1702744},
    eprint = {https://pubs.aip.org/aip/jap/article-pdf/34/8/2346/18329547/2346\_1\_online.pdf},
}

@article{Garcia_2006,
    author = {Hernando Garcia and Ramki Kalyanaraman},
    title = {Phonon-assisted two-photon absorption in the presence of a dc-field: the nonlinear {F}ranz-{K}eldysh effect in indirect gap semiconductors},
    journal = {J. Phys. B: At. Mol. Opt. Phys.},
    volume = {39},
    pages = {2737 -- 2746},
    year = {2006},
    doi = {10.1088/0953-4075/39/12/009}
}

@article{Gopal_2021,
    title = {Recent advances in nonlinear microscopy: Deep insights and polarized revelations},
    journal = {The International Journal of Biochemistry and Cell Biology},
    volume = {130},
    pages = {105896},
    year = {2021},
    issn = {1357-2725},
    doi = {https://doi.org/10.1016/j.biocel.2020.105896},
    url = {https://www.sciencedirect.com/science/article/pii/S1357272520302132},
    author = {A.A. Gopal and A. Kazarine and J.M. Dubach and P.W. Wiseman},
    keywords = {Nonlinear microscopy, Multiphoton microscopy, Harmonic generation, Imaging},
   
}

@article{Hall_2013, 
    title={Nanoscale sensing and imaging in biology using the nitrogen-vacancy center in diamond}, 
    volume={38}, 
    DOI={10.1557/mrs.2013.24}, 
    number={2}, 
    journal={MRS Bulletin}, 
    author={Hall, L.T. and Simpson, D.A. and Hollenberg, L.C.L.}, 
    year={2013}, 
    pages={162–167}
}

@article{Hausmann_2014,
    author = {B. J. M. Hausmann, I. Bulu, V. Venkataraman, P. Deotare and M. Loncar},
    journal = {nature photonics},
    number = {8},
    pages = {369--374},
    publisher = {Optica},
    title = {Diamond nonlinear photonics},
    year = {2014},
    doi = {10.1038/nphoton.2014.72},
}

@article{Ivanov_2013,
author = {Ivaylo P. Ivanov and Xiangping Li and Philip R. Dolan and Min Gu},
journal = {Opt. Lett.},
keywords = {Fluorescent and luminescent materials; Multiphoton processes; Nanomaterials; Avalanche photodiodes; Defect center materials; Nitrogen vacancy centers; Nonlinear absorption; Optical properties; Spatial resolution},
number = {8},
pages = {1358--1360},
publisher = {Optica Publishing Group},
title = {Nonlinear absorption properties of the charge states of nitrogen-vacancy centers in nanodiamonds},
volume = {38},
month = {Apr},
year = {2013},
url = {https://opg.optica.org/ol/abstract.cfm?URI=ol-38-8-1358},
doi = {10.1364/OL.38.001358},
}


@article{Ji_2018,
    author = {Peng Ji and R. Balili},
    title = {Multiple-photon excitation of nitrogen vacancy centers in diamond},
    journal = {Phys. Rev. B},
    volume = {97},
    pages = {134112},
    year = {2018},
    doi = {10.1103/PhysRevB.97.134112}
}

@article{Johnson_2025,
    author = {Johnson, Bret C. and de~Vries, Mitchell O. and Healey, Alexander J.},
    title = {The {N}itrogen-{V}acancy-{N}itrogen {C}olor {C}enter: {A U}biquitoous {V}isible and {N}ear-{I}nfrared-{II Q}uantum {E}mitter in {N}itrogen-{D}oped {D}iamond},
    journal = {ACS NANO},
    volume = {19},
    pages = {19046--19056},
    year = {2025},
    doi = {10.1021/acsnano.4c18283}
}

@article{Kolodziej_2024,
    author = {Tomasz Ko{\l}odziej and Mariusz Mr\'{o}zek and Saravanan Sengottuvel and Maciej J. G{\l}owacki and Mateusz Ficek and Wojciech Gawlik and Zenon Rajfur and Adam M. Wojciechowski},
    journal = {Biomed. Opt. Express},
    keywords = {Avalanche photodiodes; CMOS cameras; Defect center materials; Fluorescence microscopy; Green lasers; Nitrogen vacancy centers},
    number = {7},
    pages = {4024--4043},
    publisher = {Optica Publishing Group},
    title = {Multimodal analysis of traction forces and the temperature dynamics of living cells with a diamond-embedded substrate},
    volume = {15},
    month = {Jul},
    year = {2024},
    url = {https://opg.optica.org/boe/abstract.cfm?URI=boe-15-7-4024},
    doi = {10.1364/BOE.524293}
}

@article{Kozak_2012,
    author = {M. Kozak and F. Trojanek and B. Dzurnak and P. Maly},
    title = {Two- and three-photon absorption in chemical vapor deposition diamond},
    journal = {Journal of the Optical Society of America - Optical Physics},
    volume = {29},
    pages = {1141 -- 1145},
    year = {2012},
    doi = {}
}

@article{Lesik_2019,
    author = {Margarita Lesik  and Thomas Plisson  and Loïc Toraille  and Justine Renaud  and Florent Occelli  and Martin Schmidt  and Olivier Salord  and Anne Delobbe  and Thierry Debuisschert  and Loïc Rondin  and Paul Loubeyre  and Jean-François Roch },
    title = {Magnetic measurements on micrometer-sized samples under high pressure using designed NV centers},
    journal = {Science},
    volume = {366},
    number = {6471},
    pages = {1359-1362},
    year = {2019},
    doi = {10.1126/science.aaw4329},
    URL = {https://www.science.org/doi/abs/10.1126/science.aaw4329},
    eprint = {https://www.science.org/doi/pdf/10.1126/science.aaw4329},
}

@article{Levenson_1974,
    author = {Levenson, M.D. and Bloembergen, N.},
    title = {Dispersion of nonlinear optical susceptibility tensor in centrosymmetric media},
    journal = {Physical Review B},
    volume = {10},
    pages = {4447 -- 4463},
    year = {1974},
    doi = {10.1103/PhysRevB.10.4447},
}

@article{Linares_1999,
title = {Properties of large single crystal diamond},
journal = {Diamond and Related Materials},
volume = {8},
number = {2},
pages = {909-915},
year = {1999},
issn = {0925-9635},
doi = {https://doi.org/10.1016/S0925-9635(98)00382-3},
url = {https://www.sciencedirect.com/science/article/pii/S0925963598003823},
author = {Robert Linares and Patrick Doering},
keywords = {CVD, Optical properties, Single crystal diamond, Structural properties},
}

@article{Motojima_2019,
    author = {Mari Motojima and Takara Suzuki and Hidemi Shigekawa and Yuta Kainuma and Toshu An and Muneaki Hase},
    journal = {Opt. Express},
    keywords = {Nitrogen vacancy centers; Nonlinear absorption; Nonlinear effects; Nonlinear optical crystals; Optical properties; Ultrafast lasers},
    number = {22},
    pages = {32217--32227},
    publisher = {Optica Publishing Group},
    title = {Giant nonlinear optical effects induced by nitrogen-vacancy centers in diamond crystals},
    volume = {27},
    month = {Oct},
    year = {2019},
    url = {https://opg.optica.org/oe\stract.cfm?URI=oe-27-22-32217},
    doi = {10.1364/OE.27.032217},
}

@misc{mrozek,
  author = {Mariusz Mrózek and Wojciech Talik and Adam M. Wojciechowski and Krzysztof Dzierżęga},
  title = {Dataset for article: Impact of Nitrogen-Vacancy Color Centers on the Optical {K}err Effect in Diamond: A Femtosecond {Z}-Scan Study},
  year = {2025},
  doi = {https://doi.org/10.57903/UJ/E2FJ1B},
  publisher = {RODBUK},
  howpublished= {Dataset available at \url{https://doi.org/10.57903/UJ/E2FJ1B}} 
}

@article{Rand_1985,
author = {S. C. Rand and L. G. DeShazer},
journal = {Opt. Lett.},
keywords = {Laser beams; Laser crystals; Luminescence; Q switched lasers; Quantum efficiency; Solid state lasers},
number = {10},
pages = {481--483},
publisher = {Optica Publishing Group},
title = {Visible color-center laser in diamond},
volume = {10},
month = {Oct},
year = {1985},
url = {https://opg.optica.org/ol/abstract.cfm?URI=ol-10-10-481},
doi = {10.1364/OL.10.000481},
}

@article{Rand_1988,
    author = {Rand, S.C.},
    title = {Ultraviolet four-wave mixing and phase conjugation with metastable color center states in diamond},
    journal = {Optics Letters},
    volume = {13},
    number = {2},
    pages = {140--142},
    year = {1988},
    doi = {10.1364/OL.13.000140}
}

@article{Rizzato_2023,
    author = {Rizzato, Roberto and von Grafenstein, Nick R. and Bucher, Dominik B.},
    title = "{Quantum sensors in diamonds for magnetic resonance spectroscopy: Current applications and future prospects}",
    journal = {Applied Physics Letters},
    volume = {123},
    number = {26},
    pages = {260502},
    year = {2023},
    month = {12},
    issn = {0003-6951},
    doi = {10.1063/5.0169027},
    url = {https://doi.org/10.1063/5.0169027},
    eprint = {https://pubs.aip.org/aip/apl/article-pdf/doi/10.1063/5.0169027/19981024/260502\_1\_5.0169027.pdf},
}

@inbook{Rottwitt_2015,
    author    = {K. Rottwitt and P. Tidemand-Lichtenberg},
    title     = {Nonlinear Optics: Principles and Applications},
    chapter   = {4, New York},
    year      = {2015},
    publisher = {CRC},
    isbn      = {978-1-4665-6582-1}
}

@article{Seo_2011,
    author = {Seo, Jin-Gyo and Ahn, Yong-Kil and Park, Jong-Wan},
    journal = {Met Mater. Int. },
    volume = {17},    
    number = {6},
    pages = {1031--1038},
    publisher = {},
    title = {Investigation on the {O}rigin of {V}acancy {F}ormation in {D}iamonds by {E}lectron-{B}eam {I}rradiation and {H}eat-{T}reatment},
    year = {2011},
    doi = {10.1007/s112540-011-6024-6},
}

@article{Sheikbahae_1990a,
    author = {Mansoor Sheik-Bahae and Ali A. Said and T. H. Wei and David J. Hagan and Eric W. Van Stryland},
    title = {Sensitive measurement of optical nonlinearities using a single beam},
    journal = {IEEE J. Quant. Electron.},
    volume = {26},
    pages = {760 -- 769},
    year = {1990},
    doi = {10.1109/3.53394},
}

@article{Sheikbahae_1990b,
    author = {Mansoor Sheik-Bahae and David J. Hagan and Eric W. Van Stryland},
    title = {{Dispersion and {B}and-{G}ap {S}caling of the {E}lectronic {K}err {E}ffect in {S}olids {A}ssociated with {T}wo-{P}hoton {A}bsorption}},
    journal = {Phys. Rev. Lett.},
    volume = {65},
    number = {1},
    pages = {96 -- 99},
    year = {1990},
    doi = {},
    URL = {}
}

@article{Sheikbahae_1991,
    author = {Mansoor Sheik-Bahae and David C. Hutchinson and David J. Hagan and Eric W. Van Stryland},
    title = {{Dispersion of {B}ound {E}lectronic {N}onlinear {R}efraction in {S}olids}},
    journal = {IEEE J. Quant. Electron.},
    volume = {27},
    number = {6},
    pages = {1296 -- 1309},
    year = {1991},
    doi = {},
    URL = {}
}

@inproceedings{Sheikbahae_1995,
    author = {Mansoor Sheik-Bahae and Richard John DeSalvo and Ali A. Said and David J. Hagan and M. J. Soileau and Eric W. Van Stryland},
    title = {{Optical nonlinearities in diamond}},
    volume = {2428},
    booktitle = {Laser-Induced Damage in Optical Materials: 1994},
    editor = {Harold E. Bennett and Arthur H. Guenther and Mark R. Kozlowski and Brian Emerson Newnam and M. J. Soileau},
    organization = {International Society for Optics and Photonics},
    publisher = {SPIE},
    pages = {605 -- 609},
    year = {1995},
    doi = {10.1117/12.213706},
    URL = {https://doi.org/10.1117/12.213706}
}

@article{Shields_2015,
    title = {Efficient Readout of a Single Spin State in Diamond via Spin-to-Charge Conversion},
    author = {Shields, B. J. and Unterreithmeier, Q. P. and de Leon, N. P. and Park, H. and Lukin, M. D.},
    journal = {Phys. Rev. Lett.},
    volume = {114},
    issue = {13},
    pages = {136402},
    numpages = {5},
    year = {2015},
    month = {Mar},
    publisher = {American Physical Society},
    doi = {10.1103/PhysRevLett.114.136402},
    url = {https://link.aps.org/doi/10.1103/PhysRevLett.114.136402}
}

@article{Shinei_2022,
    author = {Shinei, Chikara and Masuyama, Yuta and Miyakawa, Masashi and Abe, Hiroshi and Ishii, Shuya and Saiki, Seiichi and Onoda, Shinobu and Taniguchi, Takashi and Ohshima, Takeshi and Teraji, Tokuyuki},
    title = "{Nitrogen related paramagnetic defects: Decoherence source of ensemble of NV- center}",
    journal = {Journal of Applied Physics},
    volume = {132},
    number = {21},
    pages = {214402},
    year = {2022},
    month = {12},
    issn = {0021-8979},
    doi = {10.1063/5.0103332},
    url = {https://doi.org/10.1063/5.0103332},
    eprint = {https://pubs.aip.org/aip/jap/article-pdf/doi/10.1063/5.0103332/16520818/214402\_1\_online.pdf},
}

@article{Solà-Garcia_2020,
author = {Solà-Garcia, Magdalena and Meuret, Sophie and Coenen, Toon and Polman, Albert},
title = {Electron-Induced State Conversion in Diamond NV Centers Measured with Pump–Probe Cathodoluminescence Spectroscopy},
journal = {ACS Photonics},
volume = {7},
number = {1},
pages = {232-240},
year = {2020},
}

@article{Talik_2025,
author = {Wojciech Talik and Mariusz Mr\'{o}zek and Adam M. Wojciechowski and Krzysztof Dzier\.{z}ęga},
journal = {Opt. Express},
keywords = {Defect center materials; Kerr effect; Nitrogen vacancy centers; Nonlinear effects; Nonlinear optics applications; Optical properties},
number = {6},
pages = {13748--13757},
publisher = {Optica Publishing Group},
title = {Impact of nitrogen-vacancy color centers on the optical Kerr effect in diamond: a femtosecond {Z}-scan study},
volume = {33},
month = {Mar},
year = {2025},
url = {https://opg.optica.org/oe/abstract.cfm?URI=oe-33-6-13748},
doi = {10.1364/OE.553603},
}

@article{Torelli_2020,
AUTHOR={Torelli, Marco D.  and Nunn, Nicholas A.  and Jones, Zachary R.  and Vedelaar, Thea  and Padamati, Sandeep Kumar  and Schirhagl, Romana  and Hamers, Robert J.  and Shames, Alexander I.  and Danilov, Evgeny O.  and Zaitsev, Alexander  and Shenderova, Olga A. },
TITLE={High Temperature Treatment of Diamond Particles Toward Enhancement of Their Quantum Properties},
JOURNAL={Frontiers in Physics},
VOLUME={Volume 8 - 2020},
YEAR={2020},
DOI={10.3389/fphy.2020.00205},
ISSN={2296-424X},
}

@article{Trojanek_2010,
    author = {F. Trojánek and K. Zídek and B. Dzurnák and M. Kozák and P. Mal},
    title = {Nonlinear optical properties of nanocrystalline diamond},
    journal = {Opt. Express},
    volume = {18},
    pages = {1349 -- 1357},
    year = {2010},
    doi = {10.1364/OE.18.001349},
}

@article{Ulbricht_2018,
title = {Excited-state lifetime of the $\mathrm{N}{\mathrm{V}}^{\ensuremath{-}}$ infrared transition in diamond},
author = {Ulbricht, Ronald and Loh, Zhi-Heng},
journal = {Phys. Rev. B},
volume = {98},
issue = {9},
pages = {094309},
numpages = {4},
year = {2018},
month = {Sep},
publisher = {American Physical Society},
doi = {10.1103/PhysRevB.98.094309},
url = {https://link.aps.org/doi/10.1103/PhysRevB.98.094309}
}

@article{Wee_2007,
author = {Wee, Tse-Luen and Tzeng, Yan-Kai and Han, Chau-Chung and Chang, Huan-Cheng and Fann, Wunshain and Hsu, Jui-Hung and Chen, Kuan-Ming and Yu, Yueh-Chung},
title = {Two-photon Excited Fluorescence of Nitrogen-Vacancy Centers in Proton-Irradiated Type Ib Diamond},
journal = {The Journal of Physical Chemistry A},
volume = {111},
number = {38},
pages = {9379-9386},
year = {2007},    
}

@article{Wong_2022,
  title = {Microscopic Study of Optically Stable Coherent Color Centers in Diamond Generated by High-Temperature Annealing},
  author = {Wong, King Cho and Ng, San Lam and Ho, Kin On and Shen, Yang and Wu, Jiahao and Lai, Kwing To and Leung, Man Yin and Leung, Wai Kuen and Dasari, Durga Bhaktavatsala Rao and Denisenko, Andrej and Wrachtrup, J\"org and Yang, Sen},
  journal = {Phys. Rev. Appl.},
  volume = {18},
  issue = {2},
  pages = {024044},
  numpages = {11},
  year = {2022},
  month = {Aug},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevApplied.18.024044},
  url = {https://link.aps.org/doi/10.1103/PhysRevApplied.18.024044}
}

@article{xu_2019,
    author = {Zhujing Xu and Zhang Yin and Qinkai Han and Tongcang Li},
    journal = {Opt. Mater. Express},
    keywords = {Defect center materials; Diffraction limit; Information processing; Nitrogen vacancy centers; Optical limiting; Quantum information},
    number = {12},
    pages = {4654--4668},
    publisher = {Optica Publishing Group},
    title = {Quantum information processing with closely-spaced diamond color centers in strain and magnetic fields},
    volume = {9},
    month = {Dec},
    year = {2019},
    url = {https://opg.optica.org/ome/abstract.cfm?URI=ome-9-12-4654},
    doi = {10.1364/OME.9.004654},
}

@article{Yuan_2020,
  title = {Charge state dynamics and optically detected electron spin resonance contrast of shallow nitrogen-vacancy centers in diamond},
  author = {Yuan, Zhiyang and Fitzpatrick, Mattias and Rodgers, Lila V. H. and Sangtawesin, Sorawis and Srinivasan, Srikanth and de Leon, Nathalie P.},
  journal = {Phys. Rev. Res.},
  volume = {2},
  issue = {3},
  pages = {033263},
  numpages = {11},
  year = {2020},
  month = {Aug},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevResearch.2.033263},
  url = {https://link.aps.org/doi/10.1103/PhysRevResearch.2.033263}
}

@article{Zhang_2011,
    title = {Coherent Nonlinear Quantum Feedback with Applications to On-Chip Quantum Optics},
    journal = {IFAC Proceedings Volumes},
    volume = {44},
    number = {1},
    pages = {2529-2534},
    year = {2011},
    note = {18th IFAC World Congress},
    issn = {1474-6670},
    doi = {https://doi.org/10.3182/20110828-6-IT-1002.03365},
    url = {https://www.sciencedirect.com/science/article/pii/S1474667016439935},
    author = {Jing Zhang and Re-Bing Wu},
}

@article{Zhang_2014,
    author = {Yaxin Zhang and Shen Qiao and Linlin Sun and Qi Wu Shi and Wanxia Huang and Ling Li and Ziqiang Yang},
    journal = {Optics Express},
    keywords = {Modulators; Metamaterials; Spectroscopy, teraherz ; Thin film devices and applications},
    number = {9},
    pages = {11070--11078},
    publisher = {Optica},
    title = {Photoinduced active terahertz metamaterials with nanostructured vanadium dioxide film deposited by sol-gel method},
    volume = {22},
    month = {May},
    year = {2014},
    url = {http://www.opticsexpress.org/abstract.cfm?URI=oe-22-9-11070},
    doi = {10.1364/OE.22.011070}
}

@article{Zhang2017,
    author = {B. Zhang and S.  Liu and X. Wu and T. Yi and Y.  Fang and J. Zhang  and Y. Song},
    title = {Ultrafast dynamics of carriers and nonlinear refractive index
        in bulk polycrystalline diamond}, 
    journal = {Optik},
    volume = {130},
    pages = {1073 -- 1079},
    year = {2017},
    doi = {10.1016/j.ijleo.2016.11.107},
}

@article{Zhao_2010,
    author = {J. Zhao and},
    title = {Measurement of third-order of nonlinear optical susceptibility of synthetic diamonds},
    journal = {Chinese Optics Letters},
    volume = {8},
    pages = {685 -- 688},
    year = {2010},
    doi = {10.3788/col20100807.0685}
}
